Hybrid LMC: Hybrid Learning and Model-based Control for Wheeled Humanoid Robot via Ensemble Deep Reinforcement Learning

Control of wheeled humanoid locomotion is a challenging problem due to the nonlinear dynamics and under-actuated characteristics of these robots. Traditionally, feedback controllers have been utilized for stabilization and locomotion. However, these methods are often limited by the fidelity of the underlying model used, choice of controller, and environmental variables considered (surface type, ground inclination, etc). Recent advances in reinforcement learning (RL) offer promising methods to tackle some of these conventional feedback controller issues, but require large amounts of interaction data to learn. Here, we propose a hybrid learning and model-based controller Hybrid LMC that combines the strengths of a classical linear quadratic regulator (LQR) and ensemble deep reinforcement learning. Ensemble deep reinforcement learning is composed of multiple Soft Actor-Critic (SAC) and is utilized in reducing the variance of RL networks. By using a feedback controller in tandem the network exhibits stable performance in the early stages of training. As a preliminary step, we explore the viability of Hybrid LMC in controlling wheeled locomotion of a humanoid robot over a set of different physical parameters in MuJoCo simulator. Our results show that Hybrid LMC achieves better performance compared to other existing techniques and has increased sample efficiency

==> Conclusion.tex <==
\section{Conclusion}
\label{concl}
In this paper, we propose a hybrid learning and model-based controller, \emph{Hybrid LMC}, that combines the strength of a conventional model-based LQR and deep reinforcement learning for more robust tracking in the presence of model uncertainty and parameter changes. Moreover, the ensemble deep reinforcement approach can augment the performance of a standard controller while reducing the variance of a single stochastic-based RL policy. In this manner we are able to perform end-to-end learning directly. By incorporating the ensemble deep RL and the LQR controller, LQR guides the RL policy in generating more appropriate torque within a bounded range, and results in an increase in the sampling efficiency. The ablation studies were conducted and analyzed carefully, to offer a proper method of using \emph{Hybrid LMC}. In all experiments, \emph{Hybrid LMC} outperforms the previous methods and demonstrates generalized performance improvement in the presence of model changes and irregular desired trajectories.\\
\indent In future works, we will apply \emph{Hybrid LMC} on hardware to a wheeled humanoid robot system, SATYRR, to verify the performance of \emph{Hybrid LMC} in the physical world. Based on our result, we expect that \emph{Hybrid LMC} provides an efficient way to train the real system safely while enhancing the performance.   
% \textcolor{red}{Joao: Here you could reiterate that we are going with this appraoch so we can train the system in real hardware that is inherently unstable. So exploration must be safe anda data-efficient.}

\section{Acknowledgements}
The authors are grateful to Youngwoo Sim and Guillermo Colin for their support in designing the figure and discussion for the paper. 

